Fast Nonlinear Two-Time-Scale Stochastic Approximation: Achieving $O(1/k)$ Finite-Sample Complexity

This paper proposes to develop a new variant of the two-time-scale stochastic approximation to find the roots of two coupled nonlinear operators, assuming only noisy samples of these operators can be observed. Our key idea is to leverage the classic Ruppert-Polyak averaging technique to dynamically estimate the operators through their samples. The estimated values of these averaging steps will then be used in the two-time-scale stochastic approximation updates to find the desired solution. Our main theoretical result is to show that under the strongly monotone condition of the underlying nonlinear operators the mean-squared errors of the iterates generated by the proposed method converge to zero at an optimal rate $O(1/k)$, where $k$ is the number of iterations. Our result significantly improves the existing result of two-time-scale stochastic approximation, where the best known finite-time convergence rate is $O(1/k^{2/3})$. We illustrate this result by applying the proposed method to develop new reinforcement learning algorithms with improved performance.

==> analysis.tex <==
%!TEX root = main.tex


\subsection{Convergence Results}\label{subsec:analysis}
In this section, we present the main results of this paper, which are the convergence properties of \eqref{alg:xy} under the assumptions stated in the previous section. We first study the asymptotic convergence of $(x_{k},y_{k})$ to $(x^*,y^*)$ in the following theorem. 
\begin{thm}\label{thm:asymptotic}
Suppose that Assumptions \ref{assump:smooth:FH} -- \ref{assump:noise} hold. Let $\{x_{k},y_{k}\}$ be generated by \eqref{alg:xy} with $\alpha_{k},\beta_{k}$ satisfying
\begin{align}
\begin{aligned}
&\frac{\beta_{0}}{\alpha_{0}} \leq \frac{\mu_{F}\mu_{G}}{2L_{G}},\quad \sum_{k=0}^{\infty}\alpha_{k} = \sum_{k=0}^{\infty}\beta_{k} = \infty\\  &\max\left\{\sum_{t=0}^{\infty}\alpha_{k}^2 \,\,,\sum_{t=0}^{\infty}\beta_{k}^2 \,\,,\sum_{t=0}^{\infty}\frac{\beta_{k}^2}{\alpha_{k}}\right\} < \infty.
\end{aligned}\label{thm:asymptotic:stepsizes}
\end{align}
Then we have
\begin{align}
\lim_{k\rightarrow\infty} \xhat_{k} = \lim_{k\rightarrow\infty}\yhat_{k} = 0\quad\text{a.s.} \label{thm:asymptotic:conv}   
\end{align}
\end{thm}
\begin{remark}
One can see from \eqref{thm:asymptotic:stepsizes} that $\beta_{k} \ll \alpha_{k}$. There are many choices of step sizes $\alpha_{k}$ and $\beta_{k}$ satisfying these conditions, e.g., let $1/2 < a < b\leq 1$, $2b-a>1$, and 
\begin{equation*}
\alpha_{k} = \frac{\alpha_{0}}{(k+2)^{a}},\quad \beta_{k} = \frac{\beta_{0}}{(k+2)^{b}}\cdot
\end{equation*}
In Theorem \ref{thm:rate} below, we choose $a = 2/3$ and $b = 1$ to have the best possible rate from our analysis for the convergence of the nonlinear two-time-scale SA \eqref{alg:xy}.
\end{remark}
\begin{proof}
For convenience we denote by 
\begin{equation*}
\zhat_{k} = \left[\begin{array}{c}
\xhat_{k}  \\
\yhat_{k} 
\end{array}\right].    
\end{equation*}
The main idea of our analysis is to use Lemmas \ref{lem:xhat} and \ref{lem:yhat} to show that $\|\zhat\|$ is an almost supermartingale sequence, therefore, it converges by Lemma \ref{lem:Martingale}. Indeed, adding \eqref{lem:xhat:Ineq} to \eqref{lem:yhat:Ineq} we obtain
\begin{align*}
\Eset\left[\|\zhat_{k+1}\|^2\,|\,\Qcal_{k}\right]
&\leq \left(1-\mu_{F}\alpha_{k} \right) \|\xhat_{k}\|^2 +  \beta_{k}^2\Gamma_{22} + L_{H}^2\gamma_{k}\Gamma_{22} + L_{H}^2\left(2L_{G}^2\beta_{k}^2 + \alpha_{k}^2+L_{G}^2\gamma_{k}\right)\|\xhat_{k}\|^2 \notag\\
&\quad + L_{H}^2L_{G}^2(L_{H}+1)^2\left(2\beta_{k}^2 +   \gamma_{k} \right)\|\yhat_{k}\|^2\notag\\
&\quad +  \left(1-\mu_{G}\beta_{k}\right)\|\yhat_{k}\|^2 + \beta_{k}^2\Gamma_{22} + 2L_{G}^2(L_{H}+1)^2\beta_{k}^2\|\yhat_{k}\|^2\notag\\ 
&\quad +  \frac{L_{G}\beta_{k}}{\mu_{G}}\|\xhat_{k}\|^2 +  L_{G}^2(L_{H}+2)\beta_{k}^2\|\xhat_{k}\|^2\allowdisplaybreaks\notag\\
&\leq \|\zhat_{k}\|^2 -\mu_{F}\alpha_{k}\|\xhat_{k}\|^2 - \mu_{G}\beta_{k}\|\yhat_{k}\|^2 +  \frac{L_{G}\beta_{k}}{\mu_{G}}\|\xhat_{k}\|^2 +  2\beta_{k}^2\Gamma_{22} +  \alpha_{k}^2\Gamma_{11} + L_{H}^2\gamma_{k}\Gamma_{22}\notag\\ 
&\quad + (L_{H}+1)^2\left(2L_{G}^2\beta_{k}^2 + \alpha_{k}^2+ L_{G}^2\gamma_{k}\right)\|\xhat_{k}\|^2 \notag\\
&\quad + (L_{H}^2+1)L_{G}^2(L_{H}+1)^2\left(2\beta_{k}^2 + \gamma_{k} \right)\|\yhat_{k}\|^2\allowdisplaybreaks\notag\\
&\leq \|\zhat_{k}\|^2 -\frac{\mu_{F}}{2}\alpha_{k}\|\xhat_{k}\|^2 - \mu_{G}\beta_{k}\|\yhat_{k}\|^2 +  2\beta_{k}^2\Gamma_{22} +  \alpha_{k}^2\Gamma_{11} + L_{H}^2\gamma_{k}\Gamma_{22}\notag\\
&\quad + L_{G}^2(L_{H}+1)^4\left(2L_{G}^2\beta_{k}^2 + \alpha_{k}^2 + \gamma_{k}\right)\|\zhat_{k}\|^2,
\end{align*}
where the last inequality we use \eqref{thm:asymptotic:stepsizes} to have
\begin{align*}
-\mu_{F}\alpha_{k} + \frac{L_{G}\beta_{k}}{\mu_{G}} \leq -\frac{\mu_{F}\alpha_{k}}{2}\cdot    
\end{align*}
Since $\alpha_{k},\beta_{k}$ satisfy \eqref{thm:asymptotic:stepsizes}, the relation above satisfies all the conditions in \eqref{lem:Martingale:Ineq1}, where $w_{k} = \|\zhat_{k}\|^2$. We, therefore, obtain
\begin{align*}
\left\{\begin{array}{l}
\|\zhat_{k}\|^2 = \|\xhat_{k}\|^2 + \|\yhat_{k}\|^2\; \text{ converges a.s.}  \\
    \sum_{k=0}^{\infty}  \left(\frac{\mu_{F}}{2}\alpha_{k}\|\xhat_{k}\|^2 + \mu_{G}\beta_{k}\|\yhat_{k}\|^2\right) < \infty\; \text{ a.s.}
\end{array} \right.   
\end{align*}
Since $\sum_{k=0}^{\infty} \alpha_{k} = \sum_{k=0}^{\infty} \beta_{k} = \infty$, these  relations gives \eqref{thm:asymptotic:conv}, which concludes our proof.  
\end{proof}
We next study the convergence rate of the nonlinear two-time-scale SA, where we provide a finite-time analysis for the mean square error generated by \eqref{alg:xy} to zero. The main idea is to utilize Lemmas \ref{lem:xhat}--\ref{lem:x+y_bound} and the following Lyapunov equation representing the coupling between the two iterates  
\begin{align}
V(\xhat_{k},\yhat_{k}) &= \|\yhat_{k}\|^2 + \frac{2L_{G}}{\mu_{F}\mu_{G}}\frac{\beta_{k}}{\alpha_{k}} \|\xhat_{k}\|^2\notag\\ 
&= \|y_{k} - y^{\star}\|^2 + \frac{2L_{G}}{\mu_{F}\mu_{G}}\frac{\beta_{k}}{\alpha_{k}} \|x_{k} - H(y_{k})\|^2 .\label{notation:V}    
\end{align}
The convergence rate of $V_{k}$ to zero in expectation is formally stated in the following theorem. 

\begin{thm}\label{thm:rate}
Suppose that Assumptions \ref{assump:smooth:FH} -- \ref{assump:noise} hold. Let $\{x_{k},y_{k}\}$ be generated by \eqref{alg:xy} with  $\alpha_{k},\beta_{k}$ satisfying
\begin{align}
\begin{aligned}
&\frac{\beta_{0}}{\alpha_{0}} \leq \min\left\{\frac{\mu_{F}\mu_{G}}{2L_{G}}\,,\,\frac{\mu_{F}}{2\mu_{G}}\right\},\quad \beta_{0} \geq \frac{2}{\mu_{G}},\\
&\alpha_{k} = \frac{\alpha_{0}}{(k+2)^{2/3}},\quad \beta_{k} = \frac{\beta_{0}}{(k+2)}.
\end{aligned}\label{thm:rate:stepsizes}
\end{align}
Let $D$ be defined in \eqref{lem:x+y_bound:Ineq}. Then we have for all $k\geq0$
\begin{align}
\Eset\left[V(\xhat_{k},\yhat_{k})\right]
&\leq \frac{\Eset[V(\xhat_{0},\yhat_{0})]}{(k+1)^2} + \frac{(2L_{G} + \mu_{F}\mu_{G})\beta_{0}^2\Gamma_{22} }{\mu_{F}\mu_{G}(k+1)}\notag\\ 
&\quad + \frac{4DL_{G}^2(L_{H}^2L_{G}+\mu_{F}\mu_{G})(L_{H}+1)^2\beta_{0}^2}{\mu_{F}\mu_{G}(k+1)}\notag\\
&\quad +  \frac{2L_{G}\alpha_{0}\beta_{0}\Gamma_{11}}{\mu_{F}\mu_{G}(k+1)^{2/3}} + \frac{2L_{G}L_{H}^2(1+L_{F}\alpha_{0})^2\beta_{0}^3\Gamma_{22}}{\mu_{F}^2\mu_{G}\alpha_{0}^2(k+1)^{2/3}}\notag\\
&\quad + \frac{2DL_{H}^2L_{G}(L_{H}+1)^2\beta_{0}(\alpha_{0}+ \mu_{F}\mu_{G}^2)}{\mu_{F}\mu_{G}(k+1)^{2/3}}\cdot    \label{thm:rate:ineq}
\end{align}
\end{thm}



\begin{proof}
For convenience, let $\omega_{k}$ be
\begin{equation*}
\omega_{k} = \frac{2L_{G}}{\mu_{F}\mu_{G}}\frac{\beta_{k}}{\alpha_{k}},    
\end{equation*}
which is nonincreasing due to \eqref{thm:rate:stepsizes}. The conditions in \eqref{thm:rate:stepsizes} obviously satisfy \eqref{lem:x+y_bound:stepsize}. Taking the expectation on both sides of \eqref{lem:xhat:Ineq} and multiplying both sides of \eqref{lem:xhat:Ineq} by $\omega_{k}$ we obtain
\begin{align*}
\omega_{k+1}\Eset\left[\|\xhat_{k+1}\|^2\right]
&\leq \omega_{k}\Big(1-\mu_{F}\alpha_{k} \Big) \Eset\left[\|\xhat_{k}\|^2\right]\notag\\ 
&\quad +  \frac{2L_{G}}{\mu_{F}\mu_{G}}\Big(\beta_{k}^2\Gamma_{22} +  \alpha_{k}\beta_{k}\Gamma_{11} + \frac{L_{H}^2\gamma_{k}\beta_{k}}{\alpha_{k}}\Gamma_{22}\Big)\notag\\ 
&\quad + \frac{2L_{G}L_{H}^2}{\mu_{F}\mu_{G}}\left(2L_{G}^2\beta_{k}^2 + \alpha_{k}\beta_{k} + \frac{L_{G}^2\gamma_{k}\beta_{k}}{\alpha_{k}}\right)\Eset\left[\|\xhat_{k}\|^2\right] \notag\\
&\quad + \frac{2L_{H}^2L_{G}^3(L_{H}+1)^2}{\mu_{F}\mu_{G}}\left(2\beta_{k}^2 +   \frac{\gamma_{k}\beta_{k}}{\alpha_{k}} \right)\Eset\left[\|\yhat_{k}\|^2\right]\notag\\
&= (1-\mu_{G}\beta_{k})\omega_{k} \Eset\left[\|\xhat_{k}\|^2\right] - \left(\mu_{F}\omega_{k}\alpha_{k} - \mu_{G}\beta_{k}\omega_{k}\right)\Eset\left[\|\xhat_{k}\|^2\right]\notag\\ 
&\quad +  \frac{2L_{G}}{\mu_{F}\mu_{G}}\left(\beta_{k}^2\Gamma_{22} +  \alpha_{k}\beta_{k}\Gamma_{11} + \frac{L_{H}^2\gamma_{k}\beta_{k}}{\alpha_{k}}\Gamma_{22}\right)\notag\\ 
&\quad + \frac{2L_{G}L_{H}^2}{\mu_{F}\mu_{G}}\left(2L_{G}^2\beta_{k}^2 + \alpha_{k}\beta_{k} + \frac{L_{G}^2\gamma_{k}\beta_{k}}{\alpha_{k}}\right)\Eset\left[\|\xhat_{k}\|^2\right] \notag\\
&\quad + \frac{2L_{H}^2L_{G}^3(L_{H}+1)^2}{\mu_{F}\mu_{G}}\left(2\beta_{k}^2 +   \frac{\gamma_{k}\beta_{k}}{\alpha_{k}} \right)\Eset\left[\|\yhat_{k}\|^2\right].
\end{align*}
Taking the expectation on both sides of  \eqref{lem:yhat:Ineq} and adding to the preceding relation yields 
\begin{align*}
\Eset[V(\xhat_{k+1},\yhat_{k+1})] &\leq (1-\mu_{G}\beta_{k})\Eset[V(\xhat_{k},\yhat_{k})]\notag\\ 
&\quad - \left(\mu_{F}\omega_{k}\alpha_{k} - \mu_{G}\beta_{k}\omega_{k} - \frac{L_{G}\beta_{k}}{\mu_{G}}\right)\Eset\left[\|\xhat_{k}\|^2\right]\notag\\ 
&\quad +  \frac{2L_{G}}{\mu_{F}\mu_{G}}\left(\beta_{k}^2\Gamma_{22} +  \alpha_{k}\beta_{k}\Gamma_{11} + \frac{L_{H}^2\gamma_{k}\beta_{k}}{\alpha_{k}}\Gamma_{22}\right)\notag\\ 
&\quad + \frac{2L_{G}L_{H}^2}{\mu_{F}\mu_{G}}\left(2L_{G}^2\beta_{k}^2 + \alpha_{k}\beta_{k} + \frac{L_{G}^2\gamma_{k}\beta_{k}}{\alpha_{k}}\right)\Eset\left[\|\xhat_{k}\|^2\right] \notag\\
&\quad + \frac{2L_{H}^2L_{G}^3(L_{H}+1)^2}{\mu_{F}\mu_{G}}\left(2\beta_{k}^2 +   \frac{\gamma_{k}\beta_{k}}{\alpha_{k}}\right)\Eset\left[\|\yhat_{k}\|^2\right]\notag\\
&\quad + \beta_{k}^2\Gamma_{22} + 2L_{G}^2(L_{H}+1)^2\beta_{k}^2\Eset\left[\|\yhat_{k}\|^2\right] +  L_{G}^2(L_{H}+2)\beta_{k}^2\Eset\left[\|\xhat_{k}\|^2\right],
\end{align*}
which by using \eqref{thm:rate:stepsizes} to have
\begin{align*}
 &\mu_{F}\omega_{k}\alpha_{k} - \mu_{G}\beta_{k}\omega_{k} - \frac{L_{G}\beta_{k}}{\mu_{G}} = \frac{2L_{G}\beta_{k}}{\mu_{G}} - \frac{2L_{G}}{\mu_{F}}\frac{\beta_{k}^2}{\alpha_{k}} - \frac{L_{G}\beta_{k}}{\mu_{G}} \geq 0,
\end{align*}
we obtain 
\begin{align}
\Eset[V(\xhat_{k+1},\yhat_{k+1})] &\leq (1-\mu_{G}\beta_{k})\Eset[V(\xhat_{k},\yhat_{k})] +  2L_{G}^2(L_{H}+1)^2\beta_{k}^2\Eset\left[\|\zhat_{k}\|^2\right]\notag\\ 
& +  \frac{2L_{G}}{\mu_{F}\mu_{G}}\left(\beta_{k}^2\Gamma_{22} +  \alpha_{k}\beta_{k}\Gamma_{11} + \frac{L_{H}^2\gamma_{k}\beta_{k}}{\alpha_{k}}\Gamma_{22}\right) + \beta_{k}^2\Gamma_{22}\notag\\ 
& + \frac{2L_{H}^2L_{G}^3(L_{H}+1)^2}{\mu_{F}\mu_{G}}\left(2\beta_{k}^2 + \frac{\alpha_{k}\beta_{k}}{L_{G}^2} +   \frac{\gamma_{k}\beta_{k}}{\alpha_{k}} \right)\Eset\left[\|\zhat_{k}\|^2\right]
.\label{thm:rate:eq1}
% \notag\\
% &\leq (1-\mu_{G}\beta_{k})\Eset[V(\xhat_{k},\yhat_{k})]\notag\\ 
% &\quad +  \frac{2L_{G}}{\mu_{F}\mu_{G}}\left(\beta_{k}^2\Gamma_{22} +  \alpha_{k}\beta_{k}\Gamma_{11} + \frac{L_{H}^2\gamma_{k}\beta_{k}}{\alpha_{k}}\Gamma_{22}\right) + \beta_{k}^2\Gamma_{22}\notag\\ 
% &\quad + \frac{2L_{H}^2L_{G}^3(L_{H}+1)^2}{\mu_{F}\mu_{G}}\left(\Big(2 + \frac{\mu_{F}\mu_{G}}{L_{G}L_{H}^2}\Big)\beta_{k}^2 + \frac{\alpha_{k}\beta_{k}}{L_{G}^2}  \right)\Eset\left[\|\zhat_{k}\|^2\right]\notag\\
% &\quad +  \frac{2L_{G}L_{H}^2(1+L_{F}(\Gamma_{22}+1)\alpha_{0})^2\beta_{k}^3}{\mu_{G}\mu_{F}^2\alpha_{k}^2} \left( 1  + L_{G}^2(L_{H}+1)^2 \Eset\left[\|\zhat_{k}\|^2\right]\right).\label{thm:rate:eq1}
\end{align}
Using $\gamma_{k}$ in \eqref{notation:gamma} and $\alpha_{k},\beta_{k}$ in \eqref{thm:rate:stepsizes} we have
\begin{align*}
&1.\; (k+2)^2(1-\mu_{G}\beta_{k})= (k+2)^2\left(1 - \frac{\mu_{G}\beta_{0}}{k+2}\right)\\ &\hspace{2.5cm}\leq (k+2)^2\left(1 - \frac{2}{k+2}\right) \leq (k+1)^2.\\
&2.\; (k+2)^2\alpha_{k}\beta_{k} = \alpha_{0}\beta_{0}(k+2)^{1/3}.\\
&3.\; \frac{\gamma_{k} \beta_{k}}{\alpha_{k}}(k+2)^2 \leq \frac{(1+L_{F}\alpha_{0})^2\beta_{0}^3}{\mu_{F}\alpha_{0}^2}(k+2)^{1/3}.
\end{align*}
Thus, multiplying both sides of \eqref{thm:rate:eq1} by $(k+2)^2$ and using \eqref{lem:x+y_bound:Ineq} and \eqref{thm:rate:stepsizes} we obtain 
\begin{align*}
(k+2)^2\Eset[V(\xhat_{k+1},\yhat_{k+1})]
&\leq (k+1)^2\Eset[V(\xhat_{k},\yhat_{k})] + 2L_{G}^2(L_{H}+1)^2\beta_{0}^2\Eset\left[\|\zhat_{k}\|^2\right] \notag\\ 
&\quad +  \frac{2L_{G}}{\mu_{F}\mu_{G}}\left(\beta_{0}^2\Gamma_{22} +  \alpha_{0}\beta_{0}\Gamma_{11}(k+2)^{1/3}\right) + \beta_{0}^2\Gamma_{22} 
\notag\\ 
&\quad + \frac{2L_{G}L_{H}^2(1+L_{F}\alpha_{0})^2\beta_{0}^3\Gamma_{22}}{\mu_{F}^2\mu_{G}\alpha_{0}^2}(k+2)^{1/3}\notag\\
&\quad + \frac{4L_{H}^2L_{G}^3(L_{H}+1)^2\beta_{0}^2}{\mu_{F}\mu_{G}}\Eset\left[\|\zhat_{k}\|^2\right]\notag\\
&\quad + \frac{2L_{H}^2L_{G}(L_{H}+1)^2\alpha_{0}\beta_{0}}{\mu_{F}\mu_{G}}(k+2)^{1/3}\Eset\left[\|\zhat_{k}\|^2\right]\notag\\
&\quad + \frac{2L_{H}^2L_{G}^3(L_{H}+1)^2(1+L_{F}\alpha_{0})^2\beta_{0}^3}{\mu_{F}^2\mu_{G}\alpha_{0}^2}(k+2)^{1/3}\Eset\left[\|\zhat_{k}\|^2\right]\notag\\
&\stackrel{\eqref{lem:x+y_bound:Ineq}}{\leq} (k+1)^2\Eset[V(\xhat_{k},\yhat_{k})] +\frac{(2L_{G} + \mu_{F}\mu_{G})\beta_{0}^2\Gamma_{22} }{\mu_{F}\mu_{G}} +  \frac{2L_{G}\alpha_{0}\beta_{0}\Gamma_{11}}{\mu_{F}\mu_{G}}(k+2)^{1/3} 
\notag\\ 
&\quad + \frac{2L_{G}L_{H}^2(1+L_{F}\alpha_{0})^2\beta_{0}^3\Gamma_{22}}{\mu_{F}^2\mu_{G}\alpha_{0}^2}(k+2)^{1/3}\notag\\
&\quad + \frac{4DL_{G}^2(L_{H}^2L_{G}+\mu_{F}\mu_{G})(L_{H}+1)^2\beta_{0}^2}{\mu_{F}\mu_{G}}\notag\\
&\quad + \frac{2DL_{H}^2L_{G}(L_{H}+1)^2\beta_{0}(\alpha_{0}+ \mu_{F}\mu_{G}^2)}{\mu_{F}\mu_{G}}(k+2)^{1/3},
\end{align*}
where the last inequality we use $\beta_{0}/\alpha_{0} \leq \mu_{F}\mu_{G}/(2L_{G})$ in the last term. Summing up both sides over $k = 0,\ldots,K$ for some $K>0$ we obtain
\begin{align*}
(K+2)^2\Eset[V(\xhat_{K+1},\yhat_{K+1})]
&\leq \Eset[V(\xhat_{0},\yhat_{0})] +\frac{(2L_{G} + \mu_{F}\mu_{G})\beta_{0}^2\Gamma_{22} }{\mu_{F}\mu_{G}}(K+1)\notag\\ 
&\quad +  \frac{2L_{G}\alpha_{0}\beta_{0}\Gamma_{11}}{\mu_{F}\mu_{G}}(K+2)^{4/3} 
\notag\\ 
&\quad + \frac{2L_{G}L_{H}^2(1+L_{F}\alpha_{0})^2\beta_{0}^3\Gamma_{22}}{\mu_{F}^2\mu_{G}\alpha_{0}^2}(K+2)^{4/3}\notag\\
&\quad + \frac{4DL_{G}^2(L_{H}^2L_{G}+\mu_{F}\mu_{G})(L_{H}+1)^2\beta_{0}^2}{\mu_{F}\mu_{G}}(K+1)\notag\\
&\quad + \frac{2DL_{H}^2L_{G}(L_{H}+1)^2\beta_{0}(\alpha_{0}+ \mu_{F}\mu_{G}^2)}{\mu_{F}\mu_{G}}(K+2)^{4/3},    
\end{align*}
where we use the integral test to have for all $k\geq 0$ 
\begin{align*}
&\sum_{k=0}^{K}(k+2)^{1/3} \leq \frac{1}{2^{1/3}} + \int_{t=0}^{K}(t+2)^{1/3}dt\notag\\ &= \frac{1}{2^{1/3}} + \frac{3}{4}\left((K+2)^{4/3} - \frac{1}{2^{4/3}}\right) \leq (K+2)^{4/3}.
\end{align*}
Diving both sides of the equation above by $(K+2)^2$ immediately gives \eqref{thm:rate:ineq}.
\end{proof}

\begin{remark}
First, we note that this convergence rate is the same as the one in the linear case studied in \cite{Doan_two_time_SA2019,DoanR2019} and in \cite{DalalTSM2018} with convergence in high probability. On the other hand, the recent work by \cite{Kaledin_two_time_SA2020} and \cite{Dalal_Szorenyi_Thoppe_2020} improve this rate to $1/k$ by further exploiting the linear structure of the two-time-scale SA. As a result it is not obvious whether one can apply the techniques in \cite{Kaledin_two_time_SA2020,Dalal_Szorenyi_Thoppe_2020} to improve the rates of the nonlinear two-time-scale SA studied in this paper.      


Second, as observed from Eq.\ \eqref{thm:rate:eq1}, the two terms decide the rate of the two-time-scale {\sf SA} are $\beta_{k}\alpha_{k}$ and $\beta_{k}^3/\alpha_{k}^2$, which also characterize the coupling between the two iterates. Our choice of $\alpha$ and $\beta_{k}$ in the theorem is to balance these two terms, i.e., we want to achieve
\begin{align*}
\alpha_{k}\beta_{k} = \frac{\beta_{k}^3}{\alpha_{k}^2} \Rightarrow \alpha_{k}^{3} = \beta_{k}^2.      
\end{align*}
One can choose different step sizes, which will result into different decaying rates for different components in \eqref{thm:rate:ineq}. These step sizes, however, need to satisfy the conditions in \eqref{thm:asymptotic:stepsizes}. 
\end{remark}

\section{Proofs of Lemmas \ref{lem:xhat}--\ref{lem:x+y_bound}}\label{sec:preliminaries}
In this section, we provide the analysis for the results presented in Lemmas \ref{lem:xhat}--\ref{lem:x+y_bound}. 
\subsection{Proof of Lemma \ref{lem:xhat}}
Recall that $\xhat = x-H(y)$. We consider 
\begin{align*}
\xhat_{k+1} = x_{k+1} - H(y_{k+1})
&= x_{k} - \alpha_{k}F(x_{k},y_{k}) - \alpha_{k}\xi_{k} - H(y_{k+1})\notag\\
&= \xhat_{k} -  \alpha_{k}F(x_{k},y_{k}) - \alpha_{k}\xi_{k}  + H(y_{k}) - H(y_{k+1}),
\end{align*}
which implies
\begin{align}
\|\xhat_{k+1}\|^2 &= \big\|\xhat_{k}  - \alpha_{k}F(x_{k},y_{k}) - \alpha_{k}\xi_{k} + H(y_{k}) - H(y_{k+1})\big\|^2\notag\\
&= \|\xhat_{k}  - \alpha_{k}F(x_{k},y_{k})\|^2 + \left\|H(y_{k}) - H(y_{k+1}) - \alpha_{k}\xi_{k}\right\|^2\notag\\
&\quad + 2(\xhat_{k}-F(x_{k},y_{k}))^T(H(y_{k}) - H(y_{k+1}))  - 2\alpha_{k}^2\left(\xhat_{k} - \alpha_{k}F(x_{k},y_{k})\right)^T\xi_{k}. \label{lem:xhat:Eq1}
\end{align}
We next analyze each term on the right-hand side of \eqref{lem:xhat:Eq1}. First, using $F(H(y_{k}),y_{k}) = 0$ we have 
\begin{align}
\|\xhat_{k}  - \alpha_{k}F(x_{k},y_{k})\|^2 
&= \|\xhat_{k} \|^2 - 2\alpha_{k}(x_{k} - H(y_{k}) )^TF(x_{k},y_{k})  + \| \alpha_{k}F(x_{k},y_{k})\|^2\notag\\
&= \|\xhat_{k}\|^2 - 2\alpha_{k}\xhat_{k} ^T\left(F(x_{k},y_{k}) - F(H(y_{k}),y_{k})\right)\notag\\ 
&\quad  + \alpha_{k}^2\| F(x_{k},y_{k}) - F(H(y_{k}),y_{k})\|^2\notag\\
&\leq \|\xhat_{k}\|^2 - 2\mu_{F}\alpha_{k}\|\xhat_{k} \|^2 + L_{H}^2\alpha_{k}^2\|\xhat_{k} \|^2\notag\\ 
&= \left(1-2\mu_{F}\alpha_{k} + L_{H}^2\alpha_{k}^2\right) \|\xhat_{k}\|^2,\label{lem:xhat:Eq1a}
\end{align}
where the inequality is due to the strong monotone and Lispchitz continuity of $F$, i.e., Eqs.\ \eqref{assump:sm:F:ineq} and \eqref{assump:smooth:FH:ineqF}, respectively. Recall that  
\begin{align*}
\Qcal_{k} = \{x_{0},y_{0},\xi_{0},\psi_{0},\xi_{1},\psi_{1},\ldots,\xi_{k-1},\psi_{k-1}\}.
\end{align*}
We next take the conditional expectation of the second term on the right-hand side of \eqref{lem:xhat:Eq1} w.r.t $\Qcal_{k}$ and using Assumption \ref{assump:noise} to have
\begin{align}
&\Eset\left[\left\|H(y_{k}) - H(y_{k+1}) - \alpha_{k}\xi_{k}\right\|^2\,|\,\Qcal_{k}\right]\notag\\
&= \Eset\left[\left\|H(y_{k}) - H(y_{k+1})\right\|^2\,|\,\Qcal_{k} \right]  + \alpha_{k}^2\Eset\left[\left\|\xi_{k}\right\|^2\,|\,\Qcal_{k}\right]\notag\\
&\leq L_{H}^2\Eset\left[\left\|\beta_{k}G(x_{k},y_{k}) - \beta_{k}\psi_{k}\right\|^2\,|\,\Qcal_{k} \right] + \alpha_{k}^2\Eset\left[\left\|\xi_{k}\right\|^2\,|\,\Qcal_{k}\right]\notag\\
&= L_{H}^2\beta_{k}^2\left\|G(x_{k},y_{k})\right\|^2 + L_{H}^2\beta_{k}^2\Eset\left[\|\psi_{k}\|^2\,|\,\Qcal_{k}\right]  +  \alpha_{k}^2\Eset\left[\left\|\xi_{k}\right\|^2\,|\,\Qcal_{k}\right]\notag\\
&= L_{H}^2\beta_{k}^2\left\|G(x_{k},y_{k})\right\|^2 +  \beta_{k}^2\Gamma_{22} +  \alpha_{k}^2\Gamma_{11}\notag\\
&\leq 2L_{H}^2L_{G}^2\beta_{k}^2\|\xhat_{k}\|^2 + 2L_{H}^2L_{G}^2(L_{H}+1)^2\beta_{k}^2\|\yhat_{k}\|^2     +  \beta_{k}^2\Gamma_{22} +  \alpha_{k}^2\Gamma_{11}, \label{lem:xhat:Eq1b}
\end{align}
where the last inequality we use  $G(H(y^{\star}),y^{\star}) = 0$ and the Lipschitz continuity of $G$ and $H$ to obtain 
\begin{align}
\|G(x_{k},y_{k})\|^2
 &\leq 2\|G(x_{k},y_{k}) - G(H(y_{k}),y_{k})\|^2 +  2\|G(H(y_{k}),y_{k}) - G(H(y^{\star}),y^{\star})\|^2\notag\\
&\leq 2L_{G}^2\|\xhat_{k}\|^2 + 2L_{G}^2(\|H(y_{k}) - H(y^{\star})\| + \|y_{k}-y^{\star}\|^2)\notag\\
&\leq 2L_{G}^2\|\xhat_{k}\|^2 + 2L_{G}^2(L_{H}+1)^2\|\yhat_{k}\|^2.\label{lem:xhat:Eq1b1}
\end{align}
Finally, we analyze the third term by using \eqref{lem:xhat:Eq1a} and the preceding relation
\begin{align*}
&\left(\xhat_{k} - \alpha_{k}F(x_{k},y_{k})\right)^T(H(y_{k}) - H(y_{k+1}))
\leq \|\xhat_{k} - \alpha_{k}F(x_{k},y_{k})\|\|H(y_{k}) - H(y_{k+1})\|\notag\\
&\qquad\leq L_{H}\beta_{k}(\|\xhat_{k}\| + \alpha_{k}\|F(x_{k},y_{k})\|)\|G(x_{k},y_{k}) + \psi_{k}\|\notag\\ 
&\qquad= L_{H}\beta_{k}(\|\xhat_{k}\| + \alpha_{k}\|F(x_{k},y_{k}) - F(H(y_{k}),y_{k})\|) \|G(x_{k},y_{k}) + \psi_{k}\|\notag\\ 
&\qquad\leq L_{H}(1+L_{F}\alpha_{k})\beta_{k}\|\xhat_{k}\|\left(\|G(x_{k},y_{k})\| + \|\psi_{k}\|\right), 
\end{align*}
where the equality is due to $F(H(y_{k}),y_{k}) = 0$. Applying the second inequality in Eq.\ \eqref{lem:xhat:Eq1b1} to the preceding relation yields  
%
\begin{align}
&\left(\xhat_{k} - \alpha_{k}F(x_{k},y_{k})\right)^T(H(y_{k}) - H(y_{k+1}))\notag\\
&\qquad\leq L_{H}(1+L_{F}\alpha_{k})\beta_{k}\|\xhat_{k}\|\left(L_{G}\|\xhat_{k}\| + L_{G}(L_{H}+1)\|\yhat_{k}\| + \|\psi_{k}\|\right)\notag\\
&\qquad\leq \frac{\mu_{F}}{2}\alpha_{k}\|\xhat_{k}\|^2 + \gamma_{k}\left(L_{G}\|\xhat_{k}\| + L_{G}(L_{H}+1)\|\yhat_{k}\| + \|\psi_{k}\|\right)^2\notag\\
&\qquad\leq \frac{\mu_{F}}{2}\alpha_{k}\|\xhat_{k}\|^2 + 2L_{H}^2\gamma_{k} \left(L_{G}^2\|\xhat_{k}\|^2 + L_{G}^2(L_{H}+1)^2\|\yhat_{k}\|^2 + \|\psi_{k}\|^2\right),    \label{lem:xhat:Eq1c}
\end{align}
where the second inequality is due to the Cauchy-Schwarz inequality $2ab\leq \eta a^2 + 1/\eta b^2$, $\forall \eta >0$, and  $\gamma_{k}$ is defined in \eqref{notation:gamma}. Taking the conditional expectation on both sides of \eqref{lem:xhat:Eq1} w.r.t $\Qcal_{k}$ and using \eqref{lem:xhat:Eq1a}--\eqref{lem:xhat:Eq1c} and Assumption \ref{assump:noise} we obtain
\begin{align*}
\Eset\left[\|\xhat_{k+1}\|^2\,|\,\Qcal_{k}\right]
&= \left(1-2\mu_{F}\alpha_{k} \right) \|\xhat_{k}\|^2 + L_{H}^2(2L_{G}^2\beta_{k}^2 + \alpha_{k}^2)\|\xhat_{k}\|^2 \notag\\
&\quad + 2L_{H}^2L_{G}^2(L_{H}+1)^2\left(\beta_{k}^2 + 2\gamma_{k} \right)\|\yhat_{k}\|^2\notag\\
&\quad +  \beta_{k}^2\Gamma_{22} +  \alpha_{k}^2\Gamma_{11} + 4L_{H}^2\gamma_{k}\Gamma_{22} \notag\\
&\quad + \mu_{F}\alpha_{k}\|\xhat_{k}\|^2 + 4L_{H}^2L_{G}^2\gamma_{k}\|\xhat_{k}\|^2 \notag\\
&\leq \left(1-\mu_{F}\alpha_{k} \right) \|\xhat_{k}\|^2 +  \beta_{k}^2\Gamma_{22} +  \alpha_{k}^2\Gamma_{11} + 4L_{H}^2\gamma_{k}\Gamma_{22}\notag\\ 
&\quad + L_{H}^2\left(2L_{G}^2\beta_{k}^2 + \alpha_{k}^2+ 4L_{G}^2\gamma_{k}\right)\|\xhat_{k}\|^2 \notag\\
&\quad + 2L_{H}^2L_{G}^2(L_{H}+1)^2\left(\beta_{k}^2 + 2\gamma_{k} \right)\|\yhat_{k}\|^2,  
\end{align*}
which concludes our proof. 
%%%%%%%%%
%%%%%%%%%
\subsection{Proof of Lemma \ref{lem:yhat}}
Recall that $\yhat = y - y^*$. Using \eqref{alg:xy} we consider
\begin{align*}
\yhat_{k+1} &= y_{k+1} - y^{\star} = y_{k} - y^{\star} - \beta_{k}G(x_{k},y_{k})  - \beta_{k}\psi_{k} \notag\\
&= \yhat_{k} - \beta_{k}G(H(y_{k}),y_{k}) + \beta_{k} \left(G(H(y_{k}),y_{k}) - G(x_{k},y_{k})\right)  - \beta_{k}\psi_{k},
\end{align*}
which implies that
\begin{align}
\|\yhat_{k+1}\|^2 &= \|\yhat_{k} - \beta_{k}G(H(y_{k}),y_{k})\|^2 + \left\|\beta_{k} \left(G(H(y_{k}),y_{k}) - G(x_{k},y_{k})\right)  - \beta_{k}\psi_{k}\right\|^2\notag\\
&\quad + 2\beta_{k}(\yhat_{k} - \beta_{k}G(H(y_{k}),y_{k}))^T\left(G(H(y_{k}),y_{k}) - G(x_{k},y_{k})\right)\notag\\
&\quad - 2\beta_{k}(\yhat_{k} - \beta_{k}G(H(y_{k}),y_{k}))^T\psi_{k}. \label{lem:yhat:Eq1}
\end{align}
We next analyze each term on the right-hand side of \eqref{lem:yhat:Eq1}. First, using ${G(H(y^{\star}),y^{\star}) = 0}$, \eqref{assump:G:sm}, \eqref{assump:smooth:FH:ineqH} and \eqref{assump:G:smooth}  we consider the first term 
\begin{align}
\left\|\yhat_{k} - \beta_{k}G(H(y_{k}),y_{k})\right\|^2 &= \left\|\yhat_{k}\right\|^2 - 2\beta_{k}\yhat_{k}^TG(H(y_{k}),y_{k}) + \beta_{k}^2\left\|G(H(y_{k}),y_{k})\right\|^2\notag\\ 
&\leq \|\yhat_{k}\|^2 - 2\mu_{G}\beta_{k}\|\yhat_{k}\|^2  + \beta_{k}^2 \|G(H(y_{k}),y_{k}) - G(H(y^{\star}),y^{\star})\|^2\notag\\
&\leq (1- 2\mu_{G}\beta_{k})\|\yhat_{k}\|^2  + 2\beta_{k}^2 \|G(H(y_{k}),y_{k}) - G(H(y_{k}),y^{\star})\|^2\notag\\
&\quad + 2\beta_{k}^2 \| G(H(y_{k}),y^{\star}) - G(H(y^{\star}),y^{\star})\|^2\notag\\
&\leq (1- 2\mu_{G}\beta_{k})\|\yhat_{k}\|^2  + 2\beta_{k}^2 \|G(H(y_{k}),y_{k}) - G(H(y_{k}),y^{\star})\|^2\notag\\
&\quad +2\beta_{k}^2\| G(H(y_{k}),y^{\star}) - G(H(y^{\star}),y^{\star})\|^2\notag\\
&\leq (1- 2\mu_{G}\beta_{k})\|\yhat_{k}\|^2 + 2L_{G}^2\beta_{k}^2 \left(\|H(y_{k}) - H(y^{\star})\|^2 + \|\yhat_{k}\|^2\right)\notag\\
&\leq \left(1-2\mu_{G}\beta_{k} + 2(L_{H}^2+1)L_{G}^2\beta_{k}^2\right)\|\yhat_{k}\|^2.\label{lem:yhat:Eq1a}
\end{align}
Next, taking the conditional expectation of the second term on the right-hand side of \eqref{lem:yhat:Eq1} w.r.t $\Qcal_{k}$ and using Assumption \ref{assump:noise} and \eqref{assump:G:smooth} we have
\begin{align}
&\Eset\left[\left\|\beta_{k} \left(G(H(y_{k}),y_{k}) - G(x_{k},y_{k})\right)  - \beta_{k}\psi_{k}\right\|^2\;|\;\Qcal_{k}\right]\notag\\
&= \beta_{k}^2 \left\| G(H(y_{k}),y_{k}) - G(x_{k},y_{k})\right\|^2 +\beta_{k}^2 \Eset\left[\left\|\psi_{k}\right\|^2\;|\;\Qcal_{k}\right] \leq L_{G}^2\beta_{k}^2\|\xhat_{k}\|^2 + \beta_{k}^2\Gamma_{22}. 
\label{lem:yhat:Eq1b}
\end{align}
Finally, using Assumption \ref{assump:noise} and \eqref{lem:yhat:Eq1a} we consider the third term on the right-hand side of \eqref{lem:yhat:Eq1} 
\begin{align}
&2\beta_{k}(\yhat_{k} - \beta_{k}G(H(y_{k}),y_{k}))^T(G(H(y_{k}),y_{k}) - G(x_{k},y_{k})) \notag\\
&\leq 2\beta_{k}\left(\|\yhat_{k}\| + \beta_{k}\|G(H(y_{k}),y_{k})\|\right)L_{G}\|\xhat_{k}\|\notag\\
&= 2L_{G}\|\xhat_{k}\|\beta_{k}\Big(\|\yhat_{k}\| + \beta_{k}\|G(H(y_{k}),y_{k})- G(H(y_{k}),y^{\star}) + G(H(y_{k}),y^{\star}) - G(H(y^{\star}),y^{\star}) \|\Big)\notag\\
&\leq 2L_{G}(1+(L_{H}+1)L_{G}\beta_{k})\beta_{k}\|\yhat_{k}\|\|\xhat_{k}\|\notag\\
&= 2L_{G}\beta_{k}\|\yhat_{k}\|\|\xhat_{k}\| + 2L_{G}^2(L_{H}+1)\beta_{k}^2\|\yhat_{k}\|\|\xhat_{k}\|\notag\\
&\leq \mu_{G}\beta_{k}\|\yhat_{k}\|^2 + {\color{red}{\frac{L_{G}^2\beta_{k}}{\mu_{G}}}}\|\xhat_{k}\|^2 +  L_{G}^2(L_{H}+1)\beta_{k}^2(\|\yhat_{k}\|^2 + \|\xhat_{k}\|^2),\label{lem:yhat:Eq1c}
\end{align}
where the last inequality is due to the Cauchy-Schwarz inequality. Thus, taking the conditional expectation of \eqref{lem:xhat:Eq1} w.r.t $\Qcal_{k}$ and using \eqref{lem:yhat:Eq1a}--\eqref{lem:yhat:Eq1c} yields
\begin{align*}
\Eset\left[\|\yhat_{k+1}\|^2\,|\,\Qcal_{k}\right]
&\leq \left(1-2\mu_{G}\beta_{k} + 2(L_{H}^2+1)L_{G}^2\beta_{k}^2\right)\|\yhat_{k}\|^2 +  L_{G}^2\beta_{k}^2\|\xhat_{k}\|^2 \notag\\
&\quad + \beta_{k}^2\Gamma_{22} + \mu_{G}\beta_{k}\|\yhat_{k}\|^2+ \frac{L_{G}\beta_{k}}{\mu_{G}}\|\xhat_{k}\|^2\notag\\ 
&\quad  +  L_{G}^2(L_{H}+1)\beta_{k}^2(\|\yhat_{k}\|^2 + \|\xhat_{k}\|^2)\notag\\
&= \left(1-\mu_{G}\beta_{k}\right)\|\yhat_{k}\|^2 + \beta_{k}^2\Gamma_{22} + 2L_{G}^2(L_{H}+1)^2\beta_{k}^2\|\yhat_{k}\|^2\notag\\ 
&\quad + \frac{L_{G}\beta_{k}}{\mu_{G}}\|\xhat_{k}\|^2 +  L_{G}^2(L_{H}+2)\beta_{k}^2\|\xhat_{k}\|^2,
\end{align*}
which concludes our proof. 
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lem:x+y_bound}}
Let $\zhat_{k} = [\xhat_{k}^T, \yhat_{k}^T]^T$. Adding \eqref{lem:xhat:Ineq} to \eqref{lem:yhat:Ineq} yields
\begin{align}
\Eset\left[\|z_{k+1}\|^2\,|\,\Qcal_{k}\right] 
& \leq \left(1-\mu_{F}\alpha_{k} \right) \|\xhat_{k}\|^2 +  \beta_{k}^2\Gamma_{22} +  \alpha_{k}^2\Gamma_{11} + 4L_{H}^2\gamma_{k}\Gamma_{22}\notag\\ 
&\quad + L_{H}^2\left(2L_{G}^2\beta_{k}^2 + \alpha_{k}^2+ 4L_{G}^2\gamma_{k}\right)\|\xhat_{k}\|^2 \notag\\
&\quad + 2L_{H}^2L_{G}^2(L_{H}+1)^2\left(\beta_{k}^2 + 2\gamma_{k} \right)\|\yhat_{k}\|^2 + \left(1-\mu_{G}\beta_{k}\right)\|\yhat_{k}\|^2 + \beta_{k}^2\Gamma_{22}\notag\\ 
&\quad + 2L_{G}^2(L_{H}+1)^2\beta_{k}^2\|\yhat_{k}\|^2  +  \frac{L_{G}\beta_{k}}{\mu_{G}}\|\xhat_{k}\|^2 +  L_{G}^2(L_{H}+2)\beta_{k}^2\|\xhat_{k}\|^2\allowdisplaybreaks\notag\\
&\leq \|\zhat_{k}\|^2 -\mu_{G}\beta_{k}\|\yhat_{k}\|^2 - \mu_{F}\alpha_{k}\|\xhat_{k}\|^2 +  \frac{L_{G}\beta_{k}}{\mu_{G}}\|\xhat_{k}\|^2 \notag\\
&\quad +  2\beta_{k}^2\Gamma_{22} +  \alpha_{k}^2\Gamma_{11} + 4L_{G}^2\gamma_{k}\Gamma_{22}\notag\\
&\quad + 2L_{H}^2L_{G}^2(L_{H}+1)^{2}\left(\big(\frac{1}{L_{H}^2}+1\big)\beta_{k}^2 +   2\gamma_{k} \right)\|\yhat_{k}\|^2\notag\\
&\quad + L_{G}^2(L_{H}+1)^2\left(2\beta_{k}^2 + \frac{\alpha_{k}^2}{L_{G}^2} + 4\gamma_{k}\right)\|\xhat_{k}\|^2\notag\\
&\leq \|\zhat_{k}\|^2 -\mu_{G}\beta_{k}\|\yhat_{k}\|^2 - \frac{\mu_{F}}{2}\alpha_{k}\|\xhat_{k}\|^2  +  2\beta_{k}^2\Gamma_{22} +  \alpha_{k}^2\Gamma_{11} + 4L_{G}^2\gamma_{k}\Gamma_{22}\notag\\
&\quad + 2L_{G}^2(L_{H}+1)^2\left( \frac{\alpha_{k}^2}{2L_{G}^2}+ 2(L_{H}^2+1)(\gamma_{k}+\beta_{k})\right)\|\zhat_{k}\|^2.\label{lem:x+y_bound:Eq1}
\end{align}
where in the last inequality we use 
\begin{align*}
\frac{\beta_{k}}{\alpha_{k}} \leq \frac{2\mu_{F}\mu_{G}}{L_{G}}\cdot
\end{align*}
For convenience, we denote by $c_{k}$
\begin{align*}
c_{k} = 2L_{G}^2(L_{H}+1)^2\left( \frac{\alpha_{k}^2}{2L_{G}^2}+ 2(L_{H}^2+1)(\gamma_{k}+\beta_{k})\right)\|\zhat_{k}\|^2,
\end{align*}
and let $C_{2}$ be defined in \eqref{lem:x+y_bound:C}. Using the relation ${1+x\leq \exp(x)}$ for any $x\geq 0$ and since $\alpha_{k}$ and $\beta_{k}$ satisfy \eqref{lem:x+y_bound:stepsize} we have
\begin{align}
\prod_{t=k}^{\infty}\left(1+c_{t}\right) &\leq \exp\left(\sum_{t=0}^{\infty}c_{t}\right) \leq  \exp\left(C_{2}\right) < \infty.\label{lem:x+y_bound:Eq2}
\end{align}
Let $w_{k}$ be defined as 
\begin{align*}
w_{k} = \prod_{t = k}^{\infty}\left(1 + c_{t}\right)\Eset\left[\|\zhat_{k}\|^2\right]
\end{align*}
Taking the expectation both sides of \eqref{lem:x+y_bound:Eq1} and then multiplying by a finite number 
\[\prod_{t=k+1}^{\infty}\left(1 + c_{t}\right),\]
we obtain 
\begin{align*}
w_{k+1}
&\leq w_{k} +   \left(\beta_{k}^2\Gamma_{22} +  \alpha_{k}^2\Gamma_{11} + \beta_{k}^2\Gamma_{22} + 2\gamma_{k}\Gamma_{22}\right)\prod_{t=k+1}^{\infty}\left(1 + c_{t}\right)\notag\\
&\leq w_{k} +   \exp\left(C_{2}\right)\left(2\beta_{k}^2\Gamma_{22} +  \alpha_{k}^2\Gamma_{11} + 2\gamma_{k}\Gamma_{22}\right)
,    
\end{align*}
where we dropped the negative term on the right-hand side of \eqref{lem:x+y_bound:Eq1}. Summing up both sides of the preceding equation over $k = 0,\ldots,K$ for some $K>0$ yields
\begin{align}
w_{K+1}
&\leq w_{0} + \exp\left(C_{2}\right)\Big(2\Gamma_{22}\sum_{k=0}^{K}\beta_{k}^2 +  \Gamma_{11}\sum_{k=0}^{K}\alpha_{k}^2 + \Gamma_{22}\sum_{k=0}^{K}\gamma_{k}\Big)\notag\\
&\leq w_{0} + C_{1}\exp\left(C_{2}\right)\left(3\Gamma_{22} + \Gamma_{11}\right)\notag\\
&\leq C_{2}\Eset\left[\|\zhat_{0}\|^2\right] + C_{1}\exp\left(C_{2}\right)\left(3\Gamma_{22} + \Gamma_{11}\right). \label{lem:x+y_bound:Eq2b}    
\end{align}
Diving both sides of \eqref{lem:x+y_bound:Eq2b} by $\prod_{t=K+1}^{\infty}\left(1 +c_{t}\right)$ gives \eqref{lem:x+y_bound:Ineq}, i.e., 
\begin{align*}
\Eset\left[\|\zhat_{k+1}\|^2\right]
&\leq \frac{C_{2}\Eset\left[\|\zhat_{0}\|^2\right]}{\prod_{t=K+1}^{\infty}\left(1 +c_{t}\right)}  + \frac{ C_{1}\exp\left(C_{2}\right)\left(3\Gamma_{22} + \Gamma_{11}\right)}{\prod_{t=K+1}^{\infty}\left(1 +c_{t}\right)}\notag\\
&\leq \frac{ C_{2}\Eset\left[\|\zhat_{0}\|^2\right] }{\exp(-C_{2})} + \frac{ C_{1}\exp\left(C_{2}\right)\left(3\Gamma_{22} + \Gamma_{11}\right)}{\exp(-C_{2})}, 
\end{align*}
where the second inequality is due to the relation $1+x\geq \exp(-x)$, $\forall x\geq 0$ and the lower bound of the integral test
\begin{align*}
\prod_{t=K+1}^{\infty}\!\!\!\left(1 +c_{t}\right) \geq \exp\big\{-\sum_{t=K+1}^{\infty}c_{t}\big\}\geq \exp\left(-C_{2}\right).
\end{align*}


==> prob.tex <==
%!TEX root = main.tex

\section{Nonlinear two-time-scale stochastic approximation}\label{sec:nonlinear_SA}

